COCO-FUNIT: Few-Shot Unsupervised Image Translation with a Content Conditioned Style Encoder

Unsupervised image-to-image translation intends to learn a mapping of an image in a given domain to an analogous image in a different domain, without explicit supervision of the mapping. Few-shot unsupervised image-to-image translation further attempts to generalize the model to an unseen domain by leveraging example images of the unseen domain provided at inference time. While remarkably successful, existing few-shot image-to-image translation models find it difficult to preserve the structure of the input image while emulating the appearance of the unseen domain, which we refer to as the content loss problem. This is particularly severe when the poses of the objects in the input and example images are very different. To address the issue, we propose a new few-shot image translation model, COCO-FUNIT, which computes the style embedding of the example images conditioned on the input image and a new module called the constant style bias. Through extensive experimental validations with comparison to the state-of-the-art, our model shows effectiveness in addressing the content loss problem. For code and pretrained models, please check out https://nvlabs.github.io/COCO-FUNIT/ .

==> setup.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imgs/overview.pdf}
    \caption{Problem setting in few-shot image-to-image translation. \textbf{Training.} The training dataset consists of many categories of images. We train a model to translate between the training classes. \textbf{Deployment.} We apply the trained model to perform a few-shot image translation. Given a few examples from a test class, we aim to translate a content image into an image analogous to the test class.}
    \label{fig:setting}
\end{figure*}
